Binaries masses and luminosities with Gaia DR3

The recent Gaia third data release (DR3) has brought some new exciting data about stellar binaries. It provides new opportunities to fully characterize more stellar systems and contribute to enforce our global knowledge of stars behaviour. By combining the new Gaia non-single stars catalog with double-lined spectroscopic binaries (SB2), one can determine the individual masses and luminosities of the components. To fit an empirical mass-luminosity relation in the Gaia G band, lower mass stars need to be added. Those can be derived using Gaia resolved wide binaries combined with literature data. Using the BINARYS tool, we combine the astrometric non-single star solutions in the Gaia DR3 with SB2 data from two other catalogs : the 9th Catalogue of Spectroscopic Binary orbits (SB9) and APOGEE. We also look for low mass stars resolved in Gaia with direct imaging and Hipparcos data or literature mass fraction. The combination of Gaia astrometric non-single star solutions with double-lined spectroscopic data enabled to characterize 43 binary systems with SB9 and 13 with APOGEE. We further derive the masses of 6 low mass binaries resolved with Gaia. We then derive an empirical mass-luminosity relation in the Gaia G band down to 0.12 Msun.

==> annexes_brouillon.tex <==

\subsection{APOGEE SB2 + GAIA ASTRO}


\begin{table}[h]
    \caption{Gaia + APOGEE}
    \label{table:1}
    \centering
    \begin{tabular}{ccccccc}
    \hline \hline
        GAIA DR3 Source\_ID" & $M_1$ & $\sigma_{M1}$ & $M_2$ & $\sigma_{M2}$ & $\beta$ & $\sigma_{\beta}$ \\ \hline \hline
        683525873153063680 & 0.518 & 0.202 & 0.486 & 0.198 & 0.398 & 0.042 \\
        702393458327135360 & 1.547 & 0.367 & 1.454 & 0.364 & 0.39 & 0.049 \\
        790545256897189760 & 0.437 & 0.206 & 0.374 & 0.172 & 0.289 & 0.091 \\
        794359875050204544 & 1.136 & 0.278 & 1.002 & 0.245 & 0.265 & 0.136 \\
        824315485231630592 & 0.94 & 0.231 & 0.857 & 0.246 & 0.313 & 0.336 \\
        839401128363085568 & 1.494 & 0.296 & 1.338 & 0.278 & 0.401 & 0.068 \\
        901170214141646592 & 0.924 & 0.269 & 0.775 & 0.25 & 0.232 & 0.177 \\
        1267970076306377344 & 1.171 & 0.177 & 0.776 & 0.121 & 0.073 & 0.214 \\
%        !!! 1292654730826968448 !!! & 515.435 & 214.415 & 280.486 & 138.614 & 0.336 & 0.051 \\
        !! beta !! 1390612970523119104 & 0.635 & 0.339 & 0.505 & 0.394 & 0.105 & 1.512 \\
%        !!! 1466122133423051136 !!! & 23.422 & 0.129 & 21.713 & 0.123 & 0.392 & 0.021 \\
        !! beta !! 1560143713473045248 & 0.805 & 0.397 & 0.663 & 0.367 & 0.161 & 0.782 \\
        1636132061580415488 & 1.122 & 0.375 & 0.805 & 0.326 & 0.149 & 0.299 \\
%        !!! 2080263497110638336 !!! & 35.606 & 0.24 & 10.255 & 0.458 & 0.249 & 0.464 \\
        !!! 2080409972675371008 !!! & 0.234 & 0.064 & 0.364 & 0.099 & 0.436 & 0.06 \\
        2134829544776833280 & 0.874 & 0.142 & 0.674 & 0.109 & 0.149 & 0.17 \\
        2223557418716157952 & 0.37 & 0.131 & 0.22 & 0.103 & 0.038 & 0.086 \\
        2705239237909520128 & 0.236 & 0.293 & 0.125 & 0.264 & 0.2 & 0.213 \\
        !!! 3381715240071726592 !!! & 0.52 & 0.197 & 0.569 & 0.237 & 0.264 & 0.077 \\
        !!! 3847995791877023104 !!! & 0.962 & 0.166 & 1.148 & 0.181 & 0.405 & 0.068 \\
% erreur sur beta < 0 ?        !!! 4382179737978845824 !!! & 18.985 & 0.155 & 2.122 & 0.414 & -0.085 & -0.415 \\
%        !!! 4651978450988813952 !!! & 8.617 & 3.779 & 4.359 & 1.68 & 0.186 & 0.048 \\
        4690818012020664192 & 0.235 & 0.036 & 0.212 & 0.039 & 0.325 & 0.029 \\
        !!! 5285071954833306368 !!! & 0.388 & 0.091 & 0.491 & 0.113 & 0.272 & 0.041 \\ \hline
    \end{tabular}
\end{table}

!!! = étoiles à vérifier (solution != K1<->K2, soit UNIQUE pour celle a 500 Msol et OTHER  pour les autres, celle à 8 Msol est K1<->K2 mais elle est complètement perdue sur le diagramme masse-luminosité...)



\newpage
coucou

\newpage

\begin{table}[!ht]
    \caption{Gaia + APOGEE V2}
    \label{table:1}
    \centering
    \begin{tabular}{cccccccc}
    \hline \hline
        GAIA DR3 Source\_ID" & $M_1$ & $\sigma_{M1}$ & $M_2$ & $\sigma_{M2}$ & $\beta$ & $\sigma_{\beta}$ & $F2$ \\ \hline \hline
        683525873153063680 & 0.518 & 0.105 & 0.486 & 0.096 & 0.398 & 0.017 & 1.762 \\
        702393458327135360 & 1.547 & 0.567 & 1.454 & 0.529 & 0.39 & 0.019 & !! 4.575 !! \\
        790545256897189760 & 0.437 & 0.09 & 0.374 & 0.064 & 0.289 & 0.026 & 0.717 \\
        794359875050204544 & 1.136 & 0.316 & 1.002 & 0.245 & 0.265 & 0.036 & 0.822 \\
        824315485231630592 & 0.94 & 0.217 & 0.857 & 0.211 & 0.313 & 0.105 & 3.363 \\
        839401128363085568 & 1.494 & 0.443 & 1.338 & 0.372 & 0.401 & 0.027 & 2.545 \\
        901170214141646592 & 0.924 & 0.248 & 0.775 & 0.194 & 0.232 & 0.041 & 0.471 \\
        1267970076306377344 & 1.171 & 0.207 & 0.776 & 0.094 & 0.073 & 0.016 & 0.603 \\
%masses énormes        1292654730826968448 & 515.435 & 214.415 & 280.486 & 138.614 & 0.336 & 0.051 & 1.553 \\
        ! 1390612970523119104 ! & 0.635 & 0.215 & 0.505 & 0.199 & 0.105 & 0.159 & 3.383 \\
%masses trop grosses        1466122133423051136 & 21.713 & 2.668 & 23.422 & 3.03 & 0.43 & 0.01 & 5.248 \\
        ! 1560143713473045248 ! & 0.805 & 0.32 & 0.663 & 0.243 & 0.161 & 0.125 & 0.678 \\
        1636132061580415488 & 1.122 & 0.421 & 0.805 & 0.263 & 0.149 & 0.045 & 3.322 \\
%masses trop grosses        2080263497110638336 & 35.606 & 8.53 & 14.15 & 6.486 & 0.249 & 0.116 & 1.596 \\
        2080409972675371008 & 0.364 & 0.099 & 0.234 & 0.064 & 0.219 & 0.058 & 0.65 \\
        2134829544776833280 & 0.874 & 0.124 & 0.674 & 0.074 & 0.149 & 0.025 & 0.624 \\
        2223557418716157952 & 0.37 & 0.131 & 0.22 & 0.103 & 0.038 & 0.086 & !! 7.223 !! \\
        2705239237909520128 & 0.236 & 0.069 & 0.125 & 0.033 & 0.2 & 0.043 & 0.468 \\
        3381715240071726592 & 0.52 & 0.197 & 0.569 & 0.237 & 0.264 & 0.077 & !! 5.071 !! \\
        3847995791877023104 & 0.962 & 0.159 & 1.148 & 0.208 & 0.405 & 0.027 & 1.011 \\
%masses trop grosses        4382179737978845824 & 18.985 & 2.935 & 1.828 & 0.756 & -0.085 & 0.035 & 1.089 \\
%sigmaM1 gros        4651978450988813952 & 8.617 & 3.779 & 4.359 & 1.68 & 0.186 & 0.048 & 3.839 \\
        4690818012020664192 & 0.235 & 0.036 & 0.212 & 0.039 & 0.325 & 0.029 & !! 8.458 !! \\
        5285071954833306368 & 0.491 & 0.113 & 0.388 & 0.091 & 0.156 & 0.041 & 1.686 \\ \hline
    \end{tabular}
\end{table}
! = pas présent dans la table suivante MR


\newpage
coucou

\newpage


\begin{table}[!ht]
    \caption{Gaia + APOGEE V3 avec MR}
    \label{table:1}
    \centering
    \begin{tabular}{cccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID" & $MR$ & $e_{MR}$ & $M_1$ & $\sigma_{M1}$ & $M_2$ & $\sigma_{M2}$ & $\beta$ & $\sigma_{\beta}$ & $F2$ \\ \hline \hline
%M1 trop faible        197550564129488512 & 0.967 & 0.357 & 0.086 & 0.079 & 0.083 & 0.077 & 0.27 & 0.117 & 3.485 \\
        !-! 573569212819608960 !-! & 0.959 & 0.438 & 0.314 & 0.15 & 0.301 & 0.167 & 0.299 & 0.124 & 6.204 \\ 
        683525873153063680 & 0.938 & 0.05 & 0.518 & 0.105 & 0.486 & 0.096 & 0.398 & 0.017 & 1.762 \\ 
        702393458327135360 & 0.94 & 0.025 & 1.547 & 0.567 & 1.454 & 0.529 & 0.39 & 0.019 & 4.575 \\ 
%MR extrêmement faible ? sigmaM2 quasi égal à M2        703776506515951744 & 0.034 & 0.015 & 4.989 & 4.597 & 0.169 & 0.166 & -0.081 & 0.038 & 2.708 \\ 
%MR négatif        785549591454464768 & -0.291 & 1.152 & 0.947 & 1.528 & -0.276 & 1.533 & -0.146 & 2.289 & -0.475 \\ 
        790545256897189760 & 0.856 & 0.085 & 0.437 & 0.09 & 0.374 & 0.064 & 0.289 & 0.026 & 0.717 \\ 
        794359875050204544 & 0.882 & 0.13 & 1.136 & 0.316 & 1.002 & 0.245 & 0.265 & 0.036 & 0.822 \\ 
%sigmaM1 un peu gros        799184325913199872 & 0.369 & 0.109 & 11.337 & 6.152 & 4.188 & 2.179 & 0.057 & 0.067 & 2.276 \\ 
        824315485231630592 & 0.911 & 0.383 & 0.94 & 0.217 & 0.857 & 0.211 & 0.313 & 0.105 & 3.363 \\
        !-! 838671636757296128 !-! & 1.147 & 0.526 & 0.62 & 0.448 & 0.711 & 0.525 & 0.441 & 0.118 & 4.719 \\ 
%sigmaM1 trop grand        838913357516096000 & 0.718 & 0.321 & 319.072 & 163.749 & 229.085 & 123.062 & 0.396 & 0.109 & 8.9 \\ 
        839401128363085568 & 0.896 & 0.098 & 1.494 & 0.443 & 1.338 & 0.372 & 0.401 & 0.027 & 2.545 \\ 
        901170214141646592 & 0.839 & 0.113 & 0.924 & 0.248 & 0.775 & 0.194 & 0.232 & 0.041 & 0.471 \\ 
        !-! 1205451501554383232 !-! & 0.026 & 0.007 & 1.706 & 1.125 & 0.044 & 0.03 & -0.057 & 0.019 & -1.307 \\ 
        1267970076306377344 & 0.663 & 0.059 & 1.171 & 0.207 & 0.776 & 0.094 & 0.073 & 0.016 & 0.603 \\ 
        !o! 1288590244358361344 !o! & 0.834 & 0.255 & 0.753 & 0.405 & 0.628 & 0.289 & 0.293 & 0.073 & 2.53 \\ 
%masses énormes        1292654730826968448 & 0.544 & 0.119 & 515.435 & 214.415 & 280.486 & 138.614 & 0.336 & 0.051 & 1.553 \\ 
% masses énormes        1307841047990081408 & 0.015 & 0.004 & 2160.636 & 1474.909 & 32.269 & 22.839 & -0.009 & 0.006 & 7.362 \\ 
%masses trop grosses        1435855331385247616 & 0.442 & 0.081 & 29.349 & 15.172 & 12.975 & 6.832 & 0.169 & 0.046 & 0.166 \\ 
        !o! 1451546977221270144 !o! & 0.951 & 0.257 & 1.586 & 0.532 & 1.508 & 0.766 & 0.182 & 0.102 & 3.406 \\ 
%masses trop grosses        1466122133423051136 & 1.079 & 0.035 & 21.713 & 2.668 & 23.422 & 3.03 & 0.43 & 0.01 & 5.248 \\ 
        !o! 1489638183176638848 !o! & 0.403 & 0.17 & 0.453 & 0.147 & 0.183 & 0.123 & -0.004 & 0.122 & 2.837 \\ 
%masses énormes        1544736634989286272 & 0.023 & 0.003 & 1112.074 & 1001.83 & 25.706 & 22.323 & -0.045 & 0.021 & 6.081 \\ 
%masses énormes        1547861034720072576 & 0.02 & 0.003 & 4240.895 & 3072.665 & 84.945 & 61.2 & -0.002 & 0.006 & 6.214 \\ 
%masses riquiqui, grosse erreur        1553695764970517120 & 0.983 & 0.368 & 0.062 & 0.045 & 0.061 & 0.049 & -0.109 & 0.187 & 3.847 \\ 
        1636132061580415488 & 0.717 & 0.134 & 1.122 & 0.421 & 0.805 & 0.263 & 0.149 & 0.045 & 3.322 \\ 
% sigmaM1 trop gros        2080263497110638336 & 0.022 & 0.005 & 48.649 & 9.126 & 1.089 & 0.303 & -0.013 & 0.005 & 1.601 \\ 
        2080409972675371008 & 0.644 & 0.097 & 0.364 & 0.099 & 0.234 & 0.064 & 0.219 & 0.058 & 0.65 \\ 
%sigmaM2 > M2        2085670242462975488 & 0.047 & 0.013 & 1.372 & 1.638 & 0.064 & 0.077 & -0.154 & 0.079 & -1.229 \\ 
        2134829544776833280 & 0.771 & 0.068 & 0.874 & 0.124 & 0.674 & 0.074 & 0.149 & 0.025 & 0.624 \\ 
        2223557418716157952 & 0.594 & 0.151 & 0.37 & 0.131 & 0.22 & 0.103 & 0.038 & 0.086 & 7.223 \\ 
%sigmaM1 > M1        2537538116668592000 & 0.045 & 0.013 & 556.782 & 657.962 & 24.786 & 28.166 & -0.044 & 0.036 & 4.988 \\ 
        2705239237909520128 & 0.53 & 0.103 & 0.236 & 0.069 & 0.125 & 0.033 & 0.2 & 0.043 & 0.468 \\ 
%masses énormes        3217355538965040768 & 0.014 & 0.005 & 2585.702 & 1980.292 & 35.558 & 28.517 & -0.004 & 0.006 & 6.709 \\ 
        3381715240071726592 & 1.094 & 0.266 & 0.52 & 0.197 & 0.569 & 0.237 & 0.264 & 0.077 & 5.071 \\ 
%sigmaM1 énorme        3423187311140478080 & 0.018 & 0.006 & 2.204 & 1.473 & 0.039 & 0.028 & -0.159 & 0.062 & -0.761 \\ 
        3847995791877023104 & 1.192 & 0.112 & 0.962 & 0.159 & 1.148 & 0.208 & 0.405 & 0.027 & 1.011 \\ % Nb=2, OTHER but looks good
%masses trop grosses        4382179737978845824 & 0.096 & 0.041 & 18.985 & 2.935 & 1.828 & 0.756 & -0.085 & 0.035 & 1.089 \\ 
%sigmaM1 gros        4651978450988813952 & 0.506 & 0.114 & 8.617 & 3.779 & 4.359 & 1.68 & 0.186 & 0.048 & 3.839 \\ 
        4690818012020664192 & 0.902 & 0.094 & 0.235 & 0.036 & 0.212 & 0.039 & 0.325 & 0.029 & 8.458 \\ 
        !! 4813221242758872576 !! & 0.731 & 0.129 & 0.418 & !! 0.412 !! & 0.306 & 0.303 & 0.221 & 0.083 & 0.406 \\ 
%masses énormes        5179436473975316352 & 0.009 & 0.001 & 569.867 & 1142.367 & 5.363 & 10.674 & -0.055 & 0.042 & 6.794 \\ 
        5285071954833306368 & 0.792 & 0.101 & 0.491 & 0.113 & 0.389 & 0.091 & 0.156 & 0.041 & 1.686 \\ 
        !! 5484217802956945408 !! & 1.297 & 0.144 & 1.919 & !! 1.932 !! & 2.49 & 2.513 & 0.423 & 0.058 & 1.353 \\ \hline
    \end{tabular}
\end{table}
!! = pas présent dans la table précédente, pourtant inclinaison pas proche de zero...

!-! = mauvaises contraintes, pas très intéressant...

!o! = contraintes pas top, à la limite d'être intéressant...



\newpage
coucou

\newpage



Avec solution "K1/K2", filtre ; eMR/MR < 0.5, solution!=OTHER, K1 = K1, eM1/M1 < 0.5 , F2 < 5, Nbsol > 10


\begin{table}[!ht]
    \caption{Gaia + APOGEE V3 avec MR}
    \label{table:1}
    \centering
    \begin{tabular}{ccccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID & $MR$ & $\sigma_{MR}$ & $M_1$ & $\sigma_{M1}$ & $M_2$ & $\sigma_{M2}$ & $\beta$ & $\sigma_{\beta}$ & $F2$ & $\sigma_{isc}$ \\ \hline \hline
        683525873153063680 & 0.938 & 0.05 & 0.518 & 0.105 & 0.486 & 0.096 & 0.398 & 0.017 & 1.762 & 0.011 \\ 
        702393458327135360 & 0.94 & 0.025 & 1.547 & 0.567 & 1.454 & 0.529 & 0.39 & 0.019 & 4.575 & 0.007 \\ 
        790545256897189760 & 0.856 & 0.085 & 0.437 & 0.09 & 0.374 & 0.064 & 0.289 & 0.026 & 0.717 & 0.002 \\ 
        794359875050204544 & 0.882 & 0.13 & 1.136 & 0.316 & 1.002 & 0.245 & 0.265 & 0.036 & 0.822 & 0.004 \\ 
        824315485231630592 & 0.911 & 0.383 & 0.94 & 0.217 & 0.857 & 0.211 & 0.313 & 0.105 & 3.363 & 0.001 \\ 
        839401128363085568 & 0.896 & 0.098 & 1.494 & 0.443 & 1.338 & 0.372 & 0.401 & 0.027 & 2.545 & 0.008 \\ 
        901170214141646592 & 0.839 & 0.113 & 0.924 & 0.248 & 0.775 & 0.194 & 0.232 & 0.041 & 0.471 & 0.007 \\ 
        1267970076306377344 & 0.663 & 0.059 & 1.171 & 0.207 & 0.776 & 0.094 & 0.073 & 0.016 & 0.603 & 0.02 \\ 
        1636132061580415488 & 0.717 & 0.134 & 1.122 & 0.421 & 0.805 & 0.263 & 0.149 & 0.045 & 3.322 & 0.007 \\ 
        2134829544776833280 & 0.771 & 0.068 & 0.874 & 0.124 & 0.674 & 0.074 & 0.149 & 0.025 & 0.624 & 0.007 \\ 
        2705239237909520128 & 0.53 & 0.103 & 0.236 & 0.069 & 0.125 & 0.033 & 0.2 & 0.043 & 0.468 & 0.005 \\ 
        3847995791877023104 & 0.839 & 0.079 & 1.148 & 0.208 & 0.962 & 0.159 & 0.317 & 0.024 & 1.011 & 0.003 \\ 
        4651978450988813952 & 0.506 & 0.114 & 8.617 & 3.779 & 4.359 & 1.68 & 0.186 & 0.048 & 3.839 & 0.004 \\ 
        5285071954833306368 & 0.792 & 0.101 & 0.491 & 0.113 & 0.389 & 0.091 & 0.156 & 0.041 & 1.686 & 0.008 \\ \hline
    \end{tabular}
\end{table}

\begin{table}[!ht]
    \caption{Gaia + APOGEE V3 avec MR : cas 839401128363085568 (pb ecc)}
    \label{table:1bis}
    \centering
    \begin{tabular}{ccccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID & $MR$ & $\sigma_{MR}$ & $M_1$ & $\sigma_{M1}$ & $M_2$ & $\sigma_{M2}$ & $\beta$ & $\sigma_{\beta}$ & $F2$ & $\sigma_{isc}$ \\ \hline \hline
        839401128363085568 & 0.896 & 0.098 & 1.494 & 0.443 & 1.338 & 0.372 & 0.401 & 0.027 & 2.545 & 0.008 \\ 
        839401128363085568 & 0.914 & 0.099 & 0.616 & 0.115 & 0.563 & 0.091 & 0.386 & 0.027 & 3.637 & 0.005 \\ \hline
    \end{tabular}
\end{table}

!! etoile 839401128363085568 avec ecc =0 et !=0

outlayer haut à droite --> potentiellement triple ?

!! nbre de pts dispos

\newpage
coucou

\newpage


\subsection{SB9 SB2 + GAIA ASTRO}


\begin{table}[!ht]
    \caption{Gaia + SB9}
    \label{table:2}
    \centering
    \begin{tabular}{ccccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID & $M_1$ & $M_1~up$ & $M_1~low$ & $M_2$ & $M_2~up$ & $M_2~low$ & $LR$ & $LR~up$ & $LR~low$ \\ \hline \hline
        48197783694869760 & 0.994 & 1.047 & 0.949 & 0.679 & 0.709 & 0.652 & 0.112 & 0.118 & 0.106 \\
        !!! 69883417170175488 & 0.900 & 1.055 & 0.886 & 0.84 & 0.981 & 0.831 & 0.66 & 0.681 & 0.65 \\
        478996438146017280 & 0.778 & 0.872 & 0.676 & 0.717 & 0.8 & 0.622 & 0.627 & 0.636 & 0.612 \\
        544027809281308544 & 0.909 & 0.975 & 0.85 & 0.775 & 0.825 & 0.73 & 0.16 & 0.173 & 0.149 \\ 
        595390807776621824 & 0.788 & 0.798 & 0.777 & 0.695 & 0.702 & 0.686 & 0.448 & 0.453 & 0.442 \\
        827608625636174720 & 0.776 & 0.836 & 0.634 & 0.73 & 0.787 & 0.596 & 0.69 & 0.7 & 0.674 \\
        882872210352301568 & 1.007 & 1.016 & 0.999 & 0.506 & 0.509 & 0.504 & 0.026 & 0.03 & 0.022 \\
        1067685718250692352 & 1.035 & 1.059 & 1.014 & 0.919 & 0.939 & 0.901 & 0.428 & 0.439 & 0.419 \\
        1074883087005896320 & 0.641 & 0.703 & 0.566 & 0.602 & 0.667 & 0.539 & 0.657 & 0.674 & 0.637 \\
        1324699172583973248 & 1.309 & 1.362 & 1.247 & 1.154 & 1.189 & 1.11 & 0.46 & 0.47 & 0.451 \\
        !!! 1441993625629660800 !!! & 1.116 & 1.533 & 0.881 & 0.932 & 1.284 & 0.735 & 0.102 & 0.143 & 0.067 \\
        1480959875337657088 & 0.864 & 1.122 & 0.658 & 0.811 & 0.972 & 0.65 & 0.411 & 0.484 & 0.335 \\
        1517219363639758976 & 1.114 & 1.374 & 0.927 & 0.913 & 1.125 & 0.758 & 0.195 & 0.225 & 0.168 \\
        1517927895803742080 & 0.584 & 0.606 & 0.565 & 0.549 & 0.573 & 0.529 & 0.565 & 0.574 & 0.555 \\
        1615450866336763904 & 0.999 & 1.143 & 0.758 & 0.786 & 0.896 & 0.598 & 0.15 & 0.167 & 0.112 \\
        1918953867019478144 & 1.04 & 1.046 & 1.022 & 0.967 & 0.972 & 0.951 & 0.637 & 0.644 & 0.63 \\
        2012218158438964224 & 2.072 & 2.3 & 1.868 & 1.952 & 2.176 & 1.763 & 0.51 & 0.529 & 0.491 \\
        2035577729682322176 & 0.708 & 0.984 & 0.6 & 0.641 & 0.89 & 0.541 & 0.484 & 0.523 & 0.462 \\
        PB MUP < M : 2067948245320365184 & 0.839 & 0.836 & 0.787 & 0.66 & 0.664 & 0.638 & 0.181 & 0.188 & 0.181 \\
        2129771310248902016 & 0.812 & 1.119 & 0.623 & 0.693 & 0.935 & 0.538 & 0.44 & 0.477 & 0.412 \\
        2198442167969655296 & 1.021 & 1.075 & 0.975 & 0.772 & 0.801 & 0.752 & 0.255 & 0.263 & 0.247 \\
        !!! 3283823387685219328 !!! & 1.017 & 1.075 & 0.569 & 0.754 & 0.797 & 0.422 & 0.139 & 0.17 & -0.017 \\
        3312631623125272448 & 0.99 & 1.053 & 0.936 & 0.7 & 0.746 & 0.662 & 0.161 & 0.173 & 0.152 \\
        3366718833479009408 & 1.05 & 1.114 & 1.006 & 0.673 & 0.713 & 0.645 & 0.018 & 0.024 & 0.01 \\
        3536759371865789568 & 1.588 & 1.663 & 1.519 & 1.38 & 1.429 & 1.332 & 0.262 & 0.272 & 0.254 \\
        3549833939509628672 & 0.957 & 1.003 & 0.911 & 0.9 & 0.935 & 0.862 & 0.56 & 0.576 & 0.547 \\ 
        3931519127529822208 & 1.085 & 1.196 & 1.008 & 0.838 & 0.898 & 0.792 & 0.168 & 0.177 & 0.157 \\
        3935131126305835648 & 1.418 & 1.749 & 1.16 & 0.998 & 1.225 & 0.816 & 0.156 & 0.179 & 0.131 \\
        PB MUP < M : !!! 3954536956780305792 !!! & 0.553 & 0.343 & 0.093 & 0.536 & 0.318 & 0.086 & 0.506 & 0.432 & 0.249 \\
        !!! 3964895043508685312 !!! & 0.829 & 1.586 & 0.251 & 0.664 & 1.283 & 0.207 & 0.262 & 0.34 & 0.105 \\
        !!! 4228891667990334976 !!! & 1.296 & 3.238 & 0.769 & 1.113 & 2.749 & 0.662 & 0.432 & 0.519 & 0.373 \\
        4354357901908595456 & 0.76 & 0.828 & 0.699 & 0.431 & 0.453 & 0.41 & 0.068 & 0.072 & 0.063 \\
        5762455439477309440 & 0.802 & 0.877 & 0.759 & 0.646 & 0.684 & 0.616 & 0.215 & 0.226 & 0.201 \\
        6244076338858859776 & 0.776 & 0.798 & 0.751 & 0.684 & 0.704 & 0.664 & 0.415 & 0.423 & 0.41 \\ \hline
    \end{tabular}
\end{table}

!!! erreurs très asymétriques

\newpage
Ui
\newpage

Nouvelle version avec les erreurs corrélées

\begin{table}[!ht]
    \caption{Gaia + SB9 V2}
    \label{table:2}
    \centering
    \begin{tabular}{cccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID & $M_1$ & $M_1~up$ & $M_1~low$ & $M_2$ & $M_2~up$ & $M_2~low$ & $LR$ & $LR~up$ & $LR~low$ \\ \hline \hline
        48197783694869760 & 1.026 & 1.082 & 0.975 & 0.701 & 0.734 & 0.67 & 0.116 & 0.123 & 0.11 \\
        69883417170175488 & 0.892 & 0.917 & 0.85 & 0.834 & 0.856 & 0.797 & 0.66 & 0.673 & 0.645 \\
        478996438146017280 & 0.772 & 0.797 & 0.736 & 0.711 & 0.733 & 0.678 & 0.626 & 0.633 & 0.617 \\
        544027809281308544 & 0.892 & 0.952 & 0.848 & 0.763 & 0.801 & 0.727 & 0.158 & 0.168 & 0.148 \\
        595390807776621824 & 0.763 & 0.782 & 0.742 & 0.672 & 0.688 & 0.655 & 0.444 & 0.45 & 0.438 \\
        827608625636174720 & 0.74 & 0.775 & 0.686 & 0.697 & 0.73 & 0.644 & 0.686 & 0.695 & 0.674 \\
        882872210352301568 & 1.006 & 1.016 & 0.995 & 0.506 & 0.509 & 0.502 & 0.026 & 0.03 & 0.022 \\
        1067685718250692352 & 0.985 & 1.028 & 0.935 & 0.875 & 0.913 & 0.83 & 0.422 & 0.434 & 0.408 \\
        1074883087005896320 & 0.628 & 0.665 & 0.594 & 0.59 & 0.625 & 0.558 & 0.654 & 0.674 & 0.633 \\
        1324699172583973248 & 1.307 & 1.371 & 1.245 & 1.152 & 1.204 & 1.102 & 0.458 & 0.466 & 0.45 \\
        1441993625629660800 & 1.117 & 1.157 & 1.064 & 0.933 & 0.955 & 0.9 & 0.102 & 0.11 & 0.093 \\
        1480959875337657088 & 0.859 & 1.128 & 0.641 & 0.807 & 0.994 & 0.648 & 0.409 & 0.479 & 0.35 \\
        1517219363639758976 & 1.072 & 1.122 & 1.025 & 0.879 & 0.917 & 0.842 & 0.19 & 0.199 & 0.181 \\
        1517927895803742080 & 0.604 & 0.626 & 0.583 & 0.568 & 0.592 & 0.546 & 0.568 & 0.578 & 0.558 \\
        1615450866336763904 & 1 & 1.049 & 0.955 & 0.787 & 0.822 & 0.756 & 0.151 & 0.158 & 0.144 \\
        1918953867019478144 & 1.041 & 1.09 & 0.992 & 0.968 & 1.013 & 0.923 & 0.638 & 0.645 & 0.63 \\
        2012218158438964224 & 1.72 & 1.933 & 1.513 & 1.62 & 1.819 & 1.433 & 0.49 & 0.509 & 0.469 \\
        2035577729682322176 & 0.716 & 0.786 & 0.645 & 0.648 & 0.71 & 0.583 & 0.485 & 0.498 & 0.469 \\
        --> 2067948245320365184 & 0.831 & 0.835 & 0.776 & 0.654 & 0.665 & 0.63 & 0.181 & 0.188 & 0.18 \\
        2129771310248902016 & 0.775 & 0.89 & 0.751 & 0.688 & 0.738 & 0.65 & 0.461 & 0.456 & 0.424 \\
        2198442167969655296 & 1.081 & 1.141 & 1.023 & 0.817 & 0.855 & 0.78 & 0.264 & 0.272 & 0.254 \\
        3283823387685219328 & 0.603 & 1.211 & 0.125 & 0.447 & 0.897 & 0.093 & 0.07 & 0.172 & -0.157 \\
        3312631623125272448 & 1.098 & 1.204 & 1.006 & 0.776 & 0.851 & 0.711 & 0.173 & 0.189 & 0.157 \\
        3366718833479009408 & 1.09 & 1.111 & 1.07 & 0.699 & 0.711 & 0.687 & 0.022 & 0.028 & 0.017 \\
        3536759371865789568 & 1.605 & 1.683 & 1.533 & 1.394 & 1.447 & 1.346 & 0.264 & 0.273 & 0.254 \\
        3549833939509628672 & 1.018 & 1.082 & 0.956 & 0.957 & 1.012 & 0.9 & 0.565 & 0.583 & 0.547 \\
        3931519127529822208 & 1.104 & 1.181 & 1.025 & 0.852 & 0.885 & 0.816 & 0.171 & 0.177 & 0.165 \\
        3935131126305835648 & 1.423 & 1.524 & 1.336 & 1.001 & 1.072 & 0.94 & 0.154 & 0.163 & 0.146 \\
        --> 3954536956780305792 & 0.752 & 1.126 & 0.324 & 0.729 & 1.052 & 0.302 & 0.541 & 0.586 & 0.417 \\
        3964895043508685312 & 0.753 & 1.008 & 0.614 & 0.636 & 0.824 & 0.501 & 0.262 & 0.294 & 0.231 \\
        4228891667990334976 & 1.339 & 1.426 & 1.222 & 1.142 & 1.216 & 1.046 & 0.437 & 0.445 & 0.425 \\
        4354357901908595456 & 0.77 & 0.844 & 0.702 & 0.436 & 0.461 & 0.413 & 0.069 & 0.074 & 0.064 \\
        5762455439477309440 & 0.757 & 0.829 & 0.679 & 0.609 & 0.654 & 0.562 & 0.207 & 0.222 & 0.192 \\
        6244076338858859776 & 0.768 & 0.785 & 0.751 & 0.677 & 0.69 & 0.663 & 0.414 & 0.419 & 0.409 \\ \hline
    \end{tabular}
\end{table}

\newpage
Ui
\newpage

Nouvelle version avec les erreurs corrélées + moy pondérée sur P et ecc
\begin{table}[!ht]
    \caption{Gaia + SB9 V3}
    \label{table:2}
    \centering
    \begin{tabular}{cccccccccc}
    \hline
        GAIA DR3 Source\_ID & $M_1$ & $M_1~up$ & $M_1~low$ & $M_2$ & $M_2~up$ & $M_2~low$ & $LR$ & $LR~up$ & $LR~low$ \\ \hline \hline
        48197783694869760 & 0.994 & 1.032 & 0.959 & 0.679 & 0.702 & 0.659 & 0.112 & 0.117 & 0.108 \\
        69883417170175488 & 0.899 & 0.926 & 0.875 & 0.841 & 0.864 & 0.82 & 0.66 & 0.675 & 0.646 \\
        478996438146017280 & 0.778 & 0.798 & 0.752 & 0.717 & 0.733 & 0.693 & 0.627 & 0.636 & 0.618 \\
        544027809281308544 & 0.906 & 0.965 & 0.861 & 0.773 & 0.809 & 0.742 & 0.16 & 0.169 & 0.151 \\
        595390807776621824 & 0.788 & 0.799 & 0.777 & 0.695 & 0.702 & 0.688 & 0.448 & 0.454 & 0.443 \\
        827608625636174720 & 0.776 & 0.821 & 0.724 & 0.73 & 0.77 & 0.683 & 0.69 & 0.7 & 0.68 \\ 
        882872210352301568 & 1.007 & 1.018 & 0.997 & 0.506 & 0.509 & 0.503 & 0.026 & 0.03 & 0.022 \\ 
        1067685718250692352 & 1.035 & 1.05 & 1.023 & 0.919 & 0.932 & 0.909 & 0.428 & 0.44 & 0.417 \\ 
        1074883087005896320 & 0.641 & 0.682 & 0.606 & 0.602 & 0.638 & 0.569 & 0.657 & 0.677 & 0.636 \\ 
        1324699172583973248 & 1.309 & 1.369 & 1.256 & 1.154 & 1.201 & 1.111 & 0.46 & 0.468 & 0.452 \\ 
        1441993625629660800 & 1.116 & 1.153 & 1.061 & 0.932 & 0.954 & 0.897 & 0.102 & 0.109 & 0.092 \\ 
        1480959875337657088 & 0.864 & 1.116 & 0.644 & 0.811 & 0.991 & 0.652 & 0.411 & 0.483 & 0.348 \\ 
        1517219363639758976 & 1.114 & 1.169 & 1.066 & 0.913 & 0.958 & 0.875 & 0.195 & 0.205 & 0.186 \\ 
        1517927895803742080 & 0.584 & 0.594 & 0.575 & 0.549 & 0.565 & 0.536 & 0.565 & 0.576 & 0.556 \\ 
        1615450866336763904 & 0.995 & 1.042 & 0.95 & 0.784 & 0.816 & 0.752 & 0.15 & 0.157 & 0.143 \\ 
        1918953867019478144 & 1.04 & 1.047 & 1.023 & 0.967 & 0.972 & 0.953 & 0.637 & 0.644 & 0.63 \\ 
        2012218158438964224 & 2.072 & 2.204 & 1.956 & 1.952 & 2.066 & 1.844 & 0.51 & 0.527 & 0.497 \\ 
        2035577729682322176 & 0.708 & 0.76 & 0.664 & 0.641 & 0.687 & 0.6 & 0.484 & 0.496 & 0.473 \\ 
        --> 2067948245320365184 & 0.839 & 0.832 & 0.786 & 0.66 & 0.661 & 0.64 & 0.181 & 0.188 & 0.181 \\ 
        2129771310248902016 & 0.776 & 0.886 & 0.751 & 0.688 & 0.737 & 0.649 & 0.461 & 0.456 & 0.425 \\ 
        2198442167969655296 & 1.021 & 1.066 & 0.981 & 0.772 & 0.796 & 0.749 & 0.255 & 0.262 & 0.248 \\ 
        3283823387685219328 & 1.018 & 1.119 & 0.6 & 0.754 & 0.83 & 0.445 & 0.138 & 0.172 & 0.009 \\ 
        3312631623125272448 & 0.99 & 1.08 & 0.922 & 0.7 & 0.762 & 0.652 & 0.161 & 0.178 & 0.146 \\ 
        3366718833479009408 & 1.05 & 1.062 & 1.038 & 0.673 & 0.679 & 0.667 & 0.018 & 0.023 & 0.013 \\ 
        3536759371865789568 & 1.588 & 1.665 & 1.519 & 1.38 & 1.43 & 1.333 & 0.262 & 0.272 & 0.252 \\ 
        3549833939509628672 & 0.957 & 0.992 & 0.919 & 0.9 & 0.927 & 0.872 & 0.56 & 0.577 & 0.544 \\ 
        3931519127529822208 & 1.085 & 1.164 & 1.016 & 0.838 & 0.872 & 0.807 & 0.168 & 0.174 & 0.162 \\ 
        3935131126305835648 & 1.418 & 1.508 & 1.34 & 0.998 & 1.061 & 0.942 & 0.156 & 0.163 & 0.148 \\ 
        --> 3954536956780305792 & 0.648 & 0.843 & 0.233 & 0.601 & 0.786 & 0.219 & 0.506 & 0.56 & 0.379 \\ 
        3964895043508685312 & 0.756 & 1.014 & 0.622 & 0.637 & 0.823 & 0.507 & 0.261 & 0.295 & 0.232 \\ 
        4228891667990334976 & 1.3 & 1.385 & 1.2 & 1.11 & 1.183 & 1.025 & 0.433 & 0.441 & 0.422 \\ 
        4354357901908595456 & 0.76 & 0.828 & 0.695 & 0.431 & 0.454 & 0.408 & 0.068 & 0.073 & 0.063 \\ 
        5762455439477309440 & 0.802 & 0.87 & 0.736 & 0.646 & 0.678 & 0.614 & 0.215 & 0.228 & 0.204 \\ 
        6244076338858859776 & 0.776 & 0.79 & 0.761 & 0.684 & 0.694 & 0.673 & 0.415 & 0.42 & 0.411 \\ \hline
    \end{tabular}
\end{table}

\newpage

yohoho

\newpage

CALCUL DIRECT SB9 


V4 avec sd (+ légères corrections du code)

\begin{table}[!ht]
    \centering
    \begin{tabular}{ccccccccccc}
    \hline
        source\_id & M1 & e\_M1 & M1\_up & M1\_low & M2 & e\_M2 & M2\_up & M2\_low & Lratio & e\_Lratio \\ \hline
        48197783694869760 & 0.994 & 0.036 & 1.034 & 0.962 & 0.679 & 0.021 & 0.701 & 0.66 & 0.112 & 0.004 \\ \hline
        69883417170175488 & 0.899 & 0.035 & 0.925 & 0.874 & 0.841 & 0.031 & 0.864 & 0.82 & 0.661 & 0.02 \\ \hline
        478996438146017280 & 0.778 & 0.022 & 0.797 & 0.753 & 0.717 & 0.02 & 0.733 & 0.695 & 0.627 & 0.008 \\ \hline
        544027809281308544 & 0.904 & 0.071 & 0.962 & 0.864 & 0.773 & 0.047 & 0.808 & 0.743 & 0.16 & 0.013 \\ \hline
        595390807776621824 & 0.788 & 0.01 & 0.798 & 0.778 & 0.695 & 0.007 & 0.701 & 0.688 & 0.448 & 0.005 \\ \hline
        827608625636174720 & 0.776 & 0.049 & 0.82 & 0.723 & 0.73 & 0.046 & 0.772 & 0.68 & 0.69 & 0.011 \\ \hline
        882872210352301568 & 1.007 & 0.01 & 1.017 & 0.997 & 0.506 & 0.003 & 0.509 & 0.503 & 0.026 & 0.004 \\ \hline
        1067685718250692352 & 1.035 & 0.014 & 1.05 & 1.022 & 0.919 & 0.012 & 0.932 & 0.908 & 0.428 & 0.011 \\ \hline
        1074883087005896320 & 0.641 & 0.036 & 0.678 & 0.607 & 0.602 & 0.033 & 0.637 & 0.572 & 0.657 & 0.02 \\ \hline
        1324699172583973248 & 1.309 & 0.058 & 1.373 & 1.257 & 1.154 & 0.047 & 1.205 & 1.111 & 0.46 & 0.008 \\ \hline
        1441993625629660800 & 1.116 & 0.046 & 1.157 & 1.067 & 0.932 & 0.028 & 0.955 & 0.901 & 0.102 & 0.009 \\ \hline
        1480959875337657088 & 0.864 & 0.259 & 1.148 & 0.654 & 0.811 & 0.173 & 1.008 & 0.668 & 0.411 & 0.069 \\ \hline
        1517219363639758976 & 1.114 & 0.051 & 1.163 & 1.064 & 0.913 & 0.04 & 0.953 & 0.873 & 0.195 & 0.009 \\ \hline
        1517927895803742080 & 0.584 & 0.01 & 0.595 & 0.574 & 0.549 & 0.015 & 0.565 & 0.534 & 0.565 & 0.01 \\ \hline
        1615450866336763904 & 0.995 & 0.098 & 1.045 & 0.95 & 0.784 & 0.069 & 0.818 & 0.751 & 0.15 & 0.015 \\ \hline
        1918953867019478144 & 1.04 & 0.048 & 1.047 & 1.023 & 0.967 & 0.038 & 0.972 & 0.952 & 0.637 & 0.025 \\ \hline
        2012218158438964224 & 2.072 & 0.133 & 2.218 & 1.958 & 1.952 & 0.121 & 2.085 & 1.847 & 0.51 & 0.016 \\ \hline
        2035577729682322176 & 0.708 & 0.047 & 0.752 & 0.663 & 0.641 & 0.042 & 0.68 & 0.601 & 0.484 & 0.012 \\ \hline
        --> 2067948245320365184 & 0.839 & 0.056 & 0.832 & 0.788 & 0.66 & 0.026 & 0.661 & 0.641 & 0.181 & 0.007 \\ \hline
        2129771310248902016 & 0.776 & 0.167 & 0.888 & 0.75 & 0.689 & 0.096 & 0.738 & 0.648 & 0.461 & 0.037 \\ \hline
        2198442167969655296 & 1.021 & 0.04 & 1.064 & 0.981 & 0.772 & 0.023 & 0.796 & 0.75 & 0.255 & 0.007 \\ \hline
        3283823387685219328 & 1.018 & 0.515 & 1.139 & 0.584 & 0.754 & 0.382 & 0.845 & 0.433 & 0.139 & 0.242 \\ \hline
        3312631623125272448 & 0.99 & 0.075 & 1.062 & 0.922 & 0.7 & 0.053 & 0.751 & 0.652 & 0.161 & 0.015 \\ \hline
        3366718833479009408 & 1.05 & 0.011 & 1.061 & 1.039 & 0.673 & 0.006 & 0.678 & 0.667 & 0.018 & 0.005 \\ \hline
        3536759371865789568 & 1.588 & 0.078 & 1.673 & 1.513 & 1.38 & 0.053 & 1.436 & 1.328 & 0.262 & 0.01 \\ \hline
        3549833939509628672 & 0.957 & 0.04 & 0.997 & 0.915 & 0.9 & 0.028 & 0.926 & 0.87 & 0.56 & 0.017 \\ \hline
        3931519127529822208 & 1.085 & 0.077 & 1.161 & 1.01 & 0.838 & 0.035 & 0.871 & 0.803 & 0.168 & 0.006 \\ \hline
        3935131126305835648 & 1.418 & 0.089 & 1.515 & 1.336 & 0.998 & 0.063 & 1.066 & 0.941 & 0.156 & 0.008 \\ \hline
        --> 3954536956780305792 & 0.647 & 1.987 & 0.844 & 0.238 & 0.601 & 1.908 & 0.794 & 0.223 & 0.506 & 0.126 \\ \hline
        3964895043508685312 & 0.75 & 0.332 & 1.011 & 0.618 & 0.635 & 0.266 & 0.822 & 0.504 & 0.261 & 0.046 \\ \hline
        4228891667990334976 & 1.3 & 0.139 & 1.384 & 1.194 & 1.11 & 0.117 & 1.181 & 1.019 & 0.433 & 0.014 \\ \hline
        4354357901908595456 & 0.76 & 0.137 & 0.831 & 0.695 & 0.431 & 0.046 & 0.454 & 0.408 & 0.068 & 0.01 \\ \hline
        5762455439477309440 & 0.802 & 0.069 & 0.877 & 0.737 & 0.646 & 0.033 & 0.679 & 0.613 & 0.215 & 0.012 \\ \hline
        6244076338858859776 & 0.776 & 0.015 & 0.79 & 0.761 & 0.684 & 0.01 & 0.694 & 0.674 & 0.415 & 0.005 \\ \hline
    \end{tabular}
\end{table}

\newpage
coucou
\newpage

Notes :
\begin{itemize}
    \item 1918953867019478144 --> utilise arg-periastron (gaia) au lieu de omega (sb9)
    \item 2035577729682322176 --> erreurs arbitraires fixées à 0.5 prim et 1 sec (recalcul a posteriori via methode JLH)
    \item !! 3283823387685219328 !! --> ajout de "init=list(Vr0=NSS-V0)," --> très grosses erreurs sur CD et pas sur VR --> comparer avec valeurs de JLH
    \item 3536759371865789568 --> poids 1/10 sur la secondaire
    \item 3549833939509628672 --> poids 1/5 sur la secondaire
\end{itemize}



Autres problèmes :
\begin{itemize}
    \item 69883417170175488 -->  changement de parset sur resK2
    \item 1441993625629660800 --> orbite circulaire, ecc et omega2 fixés à 0 sur la correction des erreurs
    \item 1480959875337657088 --> quasi aucun pt dans le fichier sb9, pas de recalcul des erreurs
    \item 1517927895803742080 --> 2 pt sur la secondaire, pas de recalcul des erreurs sur la secondaire resK2
    \item 3931519127529822208 --> correction des poids (1/30 pour secondaire + 1/2 pour premières obs) + nodeangle fixé (plus maintenant après le chgmt de test)
    \item 4354357901908595456 --> ajout des données Torres 2002 primary RVS
    \item 3954536956780305792 --> très grosse erreur, mais bon c'était pareil avec le calcul direct (pas accès aux données du papier...)
    \item !! 2012218158438964224 !! --> grosses erreurs, comme calcul direct, erreurs un peu plus grandes sur VR que CD et valeurs masses assez différentes
\end{itemize}



NOTES POUR MR SB9 / MODIFS APPORTEES :
\begin{itemize}
    \item 1615450866336763904 : sigma res primary = 0.196, sigma res secondary = 0.777  // données dupliquées, blended values ?
    \item 2067948245320365184 : ajout d'une colonne vide sur les premières générations de données (sinon il ne lit pas l'offset pour la dernière car ne reconnaît pas colonne supp)
    \item 2129771310248902016 : idem, ajout colonne sur premieres données
    \item 3283823387685219328 : idem, ajout colonne
    \item A quel point faut-il conserver les points "mélangés" (où les 2 composantes sont prises en compte dans la même mesure) (ex : 3549833939509628672 --> pas de résidus donnés, et pas accès aux tables de données.....). CB: enlever aussi les 2 premières lignes pas dans le papier d'origine? 
    \item 3931519127529822208 : ajustement des poids (1/30 pour la b, 1/2 pour le 1er instrument), suppression des premières données (pas de composante donnée ?)
    \item 3964895043508685312 : suppression de "-" dans la colonne V4 (car sinon, lu comme chaîne de caractères)
    \item 1517219363639758976 : 
    \item 3536759371865789568 : enlever valeurs "blended"
    \item 2012218158438964224 : idem
    
    
    \item FICHIER SB9 ORBIT : !! erreur excentricité (ex : 3283823387685219328, err = 0.000031 mais écrite à 0 sur le fichier...)
\end{itemize}


Plusieurs cas où les res intermédiaires (resK1, resK2...) convergent mieux que le res final (en terme de masse, car sinon le beta est fixé à 0)... fixer des paramètres semble être plutôt bénéfique pour les valeurs des masses ? (ex : 3536759371865789568, 3549833939509628672)\\



\newpage
coucou

\newpage

\begin{table}[!ht]
    \caption{Gaia + SB9 V4}
    \label{table:2}
    \centering
    \begin{tabular}{ccccccccc}
    \hline
        GAIA DR3 Source\_ID & $MR$ & $e_{MR}$ & $M_1$ & $e_{M1}$ & $M_2$ & $e_{M2}$ & $beta$ & $e_{beta}$ \\ \hline \hline
        "6244076338858859776" & 0.882 & 0.008 & 0.775 & 0.014 & 0.683 & 0.01 & 0.294 & 0.002 \\
        "5762455439477309440" & 0.804 & 0.033 & 0.806 & 0.067 & 0.648 & 0.033 & 0.177 & 0.008 \\
        "4354357901908595456" & 0.583 & 0.019 & 0.702 & 0.051 & 0.409 & 0.018 & 0.061 & 0.004 \\
        "4228891667990334976" & 0.863 & 0.006 & 1.097 & 0.059 & 0.946 & 0.051 & 0.288 & 0.004 \\
        "3964895043508685312" & 0.864 & 0.016 & 0.757 & 0.181 & 0.654 & 0.155 & 0.221 & 0.021 \\
        "3954536956780305792" & 0.905 & 0.009 & 0.942 & 1.033 & 0.853 & 0.935 & 0.612 & 0.059 \\
        "3935131126305835648" & 0.705 & 0.006 & 1.523 & 0.083 & 1.073 & 0.058 & 0.138 & 0.006 \\
        "3931519127529822208" & 0.775 & 0.026 & 1.079 & 0.076 & 0.836 & 0.034 & 0.14 & 0.005 \\
        "3549833939509628672" & 0.941 & 0.019 & 0.945 & 0.038 & 0.889 & 0.025 & 0.357 & 0.005 \\
        "3536759371865789568" & 0.839 & 0.022 & 1.65 & 0.093 & 1.384 & 0.051 & 0.2 & 0.006 \\
        "3366718833479009408" & 0.641 & 0.002 & 1.053 & 0.01 & 0.675 & 0.005 & 0.014 & 0.003 \\
        "3312631623125272448" & 0.706 & 0.002 & 1.014 & 0.032 & 0.716 & 0.023 & 0.128 & 0.005 \\
        "3283823387685219328" & 0.74 & 0.001 & 1.003 & 0.012 & 0.742 & 0.009 & 0.143 & 0.003 \\
        "2198442167969655296" & 0.751 & 0.015 & 0.982 & 0.042 & 0.738 & 0.019 & 0.196 & 0.003 \\
        "2129771310248902016" & 0.907 & 0.018 & 0.741 & 0.04 & 0.672 & 0.03 & 0.318 & 0.005 \\
        "2067948245320365184" & 0.786 & 0.001 & 0.836 & 0.003 & 0.657 & 0.002 & 0.151 & 0.001 \\
        "2035577729682322176" & 0.902 & 0.009 & 0.696 & 0.04 & 0.628 & 0.036 & 0.322 & 0.006 \\
        "2012218158438964224" & 0.949 & 0.015 & 2.336 & 0.164 & 2.216 & 0.151 & 0.359 & 0.006 \\
        "1918953867019478144" & 0.934 & 0.004 & 1.051 & 0.009 & 0.982 & 0.01 & 0.388 & 0.002 \\
        "1615450866336763904" & 0.786 & 0.011 & 1.008 & 0.039 & 0.793 & 0.026 & 0.131 & 0.004 \\
        "1517927895803742080" & 0.908 & 0.015 & 0.633 & 0.025 & 0.575 & 0.018 & 0.355 & 0.004 \\
        "1517219363639758976" & 0.82 & 0.006 & 1.064 & 0.04 & 0.872 & 0.031 & 0.157 & 0.007 \\
        "1480959875337657088" & 0.935 & 0.077 & 0.868 & 0.133 & 0.812 & 0.092 & 0.288 & 0.018 \\
        "1441993625629660800" & 0.834 & 0.008 & 1.105 & 0.035 & 0.922 & 0.028 & 0.056 & 0.027 \\
        "1324699172583973248" & 0.884 & 0.009 & 1.319 & 0.048 & 1.166 & 0.038 & 0.317 & 0.004 \\
        "1074883087005896320" & 0.939 & 0.026 & 0.663 & 0.039 & 0.623 & 0.033 & 0.398 & 0.007 \\
        "1067685718250692352" & 0.888 & 0.004 & 1.036 & 0.013 & 0.92 & 0.011 & 0.303 & 0.005 \\
        "882872210352301568" & 0.503 & 0.003 & 1.01 & 0.013 & 0.508 & 0.004 & 0.022 & 0.004 \\
        "827608625636174720" & 0.94 & 0.013 & 0.734 & 0.039 & 0.69 & 0.037 & 0.408 & 0.005 \\
        "595390807776621824" & 0.882 & 0.006 & 0.785 & 0.01 & 0.693 & 0.007 & 0.312 & 0.002 \\
        "544027809281308544" & 0.834 & 0.018 & 0.946 & 0.051 & 0.788 & 0.032 & 0.136 & 0.007 \\
        "478996438146017280" & 0.921 & 0.006 & 0.813 & 0.025 & 0.749 & 0.023 & 0.389 & 0.003 \\
        "69883417170175488" & 0.979 & 0.022 & 0.827 & 0.029 & 0.81 & 0.027 & 0.398 & 0.008 \\
        "48197783694869760" & 0.677 & 0.012 & 0.972 & 0.042 & 0.658 & 0.019 & 0.094 & 0.003 \\\hline
    \end{tabular}
\end{table}

\newpage

coucou

\newpage

NOUVEAUX TABLEAUX "FINAUX" SB9

CD


\begin{table*}[!ht]
    \caption{CALCUL DIRECT FINAL : Gaia + SB9}
    \label{table:2}
    \centering
    \begin{tabular}{ccccccccccccc}
    \hline
        GAIA DR3 Source\_ID & $M_1$ & $\sigma_{M1}$ & $M_{1up}$ & $M_{1low}$ & $M_{2}$ & $\sigma_{M2}$ & $M_{2up}$ & $M_{2low}$ & $LR$ & $\sigma_{LR}$ & $LR_{up}$ & $LR_{low}$ \\ \hline \hline
        48197783694869760 & 0.994 & 0.039 & 1.033 & 0.957 & 0.679 & 0.022 & 0.702 & 0.658 & 0.112 & 0.005 & 0.117 & 0.108 \\ 
        69883417170175488 & 0.895 & 0.025 & 0.921 & 0.873 & 0.843 & 0.021 & 0.865 & 0.823 & 0.665 & 0.014 & 0.679 & 0.652 \\ 
        478996438146017280 & 0.778 & 0.022 & 0.797 & 0.753 & 0.717 & 0.02 & 0.734 & 0.693 & 0.627 & 0.008 & 0.635 & 0.618 \\ 
        544027809281308544 & 0.954 & 0.053 & 1.004 & 0.902 & 0.796 & 0.033 & 0.827 & 0.764 & 0.159 & 0.009 & 0.167 & 0.151 \\ 
        595390807776621824 & 0.788 & 0.011 & 0.798 & 0.777 & 0.695 & 0.007 & 0.701 & 0.687 & 0.448 & 0.005 & 0.453 & 0.442 \\
        827608625636174720 & 0.776 & 0.052 & 0.826 & 0.726 & 0.73 & 0.049 & 0.777 & 0.683 & 0.69 & 0.01 & 0.701 & 0.68 \\ 
        882872210352301568 & 1.007 & 0.011 & 1.018 & 0.997 & 0.506 & 0.003 & 0.509 & 0.503 & 0.026 & 0.004 & 0.03 & 0.022 \\ 
        1067685718250692352 & 1.035 & 0.013 & 1.048 & 1.021 & 0.919 & 0.012 & 0.931 & 0.908 & 0.428 & 0.011 & 0.439 & 0.417 \\
        1074883087005896320 & 0.641 & 0.038 & 0.677 & 0.604 & 0.602 & 0.034 & 0.635 & 0.568 & 0.657 & 0.02 & 0.676 & 0.637 \\ 
        1324699172583973248 & 1.309 & 0.056 & 1.365 & 1.256 & 1.154 & 0.045 & 1.198 & 1.111 & 0.46 & 0.008 & 0.468 & 0.452 \\ 
        1441993625629660800 & 1.116 & 0.047 & 1.16 & 1.068 & 0.932 & 0.029 & 0.957 & 0.9 & 0.102 & 0.008 & 0.11 & 0.093 \\ 
        1480959875337657088 & 0.864 & 0.238 & 1.125 & 0.654 & 0.811 & 0.166 & 0.984 & 0.666 & 0.411 & 0.068 & 0.483 & 0.353 \\
        1517219363639758976 & 1.114 & 0.05 & 1.167 & 1.068 & 0.913 & 0.039 & 0.955 & 0.875 & 0.195 & 0.009 & 0.204 & 0.186 \\ 
        1517927895803742080 & 0.584 & 0.01 & 0.594 & 0.574 & 0.549 & 0.014 & 0.563 & 0.535 & 0.565 & 0.01 & 0.575 & 0.555 \\
        1615450866336763904 & 1 & 0.044 & 1.045 & 0.961 & 0.787 & 0.029 & 0.818 & 0.76 & 0.151 & 0.007 & 0.157 & 0.144 \\ 
        1918953867019478144 & 1.04 & 0.005 & 1.046 & 1.036 & 0.969 & 0.005 & 0.974 & 0.964 & 0.64 & 0.006 & 0.645 & 0.634 \\ 
        2012218158438964224 & 2.072 & 0.131 & 2.206 & 1.955 & 1.952 & 0.119 & 2.072 & 1.846 & 0.51 & 0.016 & 0.528 & 0.495 \\
        2035577729682322176 & 0.708 & 0.048 & 0.756 & 0.665 & 0.641 & 0.043 & 0.683 & 0.601 & 0.484 & 0.012 & 0.496 & 0.472 \\ 
        2067948245320365184 & 0.839 & 0.002 & 0.842 & 0.837 & 0.66 & 0.002 & 0.662 & 0.658 & 0.18 & 0.002 & 0.182 & 0.178 \\ 
        2129771310248902016 & 0.748 & 0.037 & 0.788 & 0.714 & 0.672 & 0.032 & 0.706 & 0.642 & 0.463 & 0.011 & 0.474 & 0.452 \\
        2198442167969655296 & 1.021 & 0.042 & 1.062 & 0.979 & 0.772 & 0.023 & 0.794 & 0.749 & 0.255 & 0.007 & 0.263 & 0.248 \\
        3283823387685219328 & 1.017 & 0.019 & 1.034 & 0.997 & 0.755 & 0.014 & 0.767 & 0.74 & 0.141 & 0.036 & 0.178 & 0.105 \\
        3312631623125272448 & 0.99 & 0.077 & 1.073 & 0.922 & 0.7 & 0.054 & 0.758 & 0.651 & 0.161 & 0.015 & 0.177 & 0.146 \\ 
        3366718833479009408 & 1.05 & 0.011 & 1.061 & 1.039 & 0.673 & 0.006 & 0.679 & 0.668 & 0.018 & 0.005 & 0.023 & 0.013 \\ 
        3536759371865789568 & 1.588 & 0.077 & 1.675 & 1.511 & 1.38 & 0.052 & 1.434 & 1.329 & 0.262 & 0.01 & 0.272 & 0.253 \\ 
        3549833939509628672 & 0.957 & 0.037 & 0.992 & 0.921 & 0.9 & 0.027 & 0.925 & 0.874 & 0.56 & 0.017 & 0.576 & 0.542 \\ 
        3931519127529822208 & 1.085 & 0.076 & 1.161 & 1.009 & 0.838 & 0.034 & 0.871 & 0.803 & 0.168 & 0.006 & 0.174 & 0.162 \\ 
        3935131126305835648 & 1.418 & 0.083 & 1.496 & 1.339 & 0.998 & 0.059 & 1.053 & 0.944 & 0.156 & 0.008 & 0.163 & 0.147 \\ 
        3954536956780305792 & 0.694 & 1.047 & 0.932 & 0.26 & 0.629 & 0.945 & 0.837 & 0.234 & 0.498 & 0.088 & 0.541 & 0.368 \\ 
        3964895043508685312 & 0.674 & 0.193 & 0.857 & 0.524 & 0.599 & 0.171 & 0.759 & 0.468 & 0.28 & 0.035 & 0.314 & 0.245 \\ 
        4228891667990334976 & 1.294 & 0.094 & 1.373 & 1.195 & 1.116 & 0.08 & 1.184 & 1.031 & 0.438 & 0.009 & 0.445 & 0.428 \\ 
        4354357901908595456 & 0.756 & 0.067 & 0.823 & 0.691 & 0.428 & 0.023 & 0.45 & 0.407 & 0.064 & 0.005 & 0.069 & 0.059 \\ 
        5762455439477309440 & 0.802 & 0.066 & 0.872 & 0.738 & 0.646 & 0.032 & 0.677 & 0.613 & 0.215 & 0.012 & 0.227 & 0.204 \\
        6244076338858859776 & 0.776 & 0.015 & 0.791 & 0.762 & 0.684 & 0.01 & 0.694 & 0.674 & 0.415 & 0.005 & 0.42 & 0.411 \\ \hline
    \end{tabular}
\end{table*}



\newpage


\begin{table*}[!ht]
    \caption{VITESSE RADIALE FINAL : Gaia + SB9}
    \label{table:2}
    \centering
    \begin{tabular}{ccccccccc}
    \hline
        GAIA DR3 Source\_ID & $MR$ & $\sigma_{MR}$ & $M_1$ & $\sigma_{M1}$ & $M_2$ & $\sigma_{M2}$ & $\beta$ & $\sigma_{\beta}$ \\ \hline \hline
        "48197783694869760" & 0.677 & 0.012 & 0.972 & 0.042 & 0.658 & 0.019 & 0.094 & 0.003 \\ 
        "69883417170175488" & 0.979 & 0.022 & 0.827 & 0.029 & 0.81 & 0.027 & 0.398 & 0.008 \\ 
        "478996438146017280" & 0.921 & 0.006 & 0.813 & 0.025 & 0.749 & 0.023 & 0.389 & 0.003 \\ 
        "544027809281308544" & 0.834 & 0.018 & 0.946 & 0.051 & 0.788 & 0.032 & 0.136 & 0.007 \\ 
        "595390807776621824" & 0.882 & 0.006 & 0.785 & 0.01 & 0.693 & 0.007 & 0.312 & 0.002 \\ 
        "827608625636174720" & 0.94 & 0.013 & 0.734 & 0.039 & 0.69 & 0.037 & 0.408 & 0.005 \\ 
        "882872210352301568" & 0.503 & 0.003 & 1.01 & 0.012 & 0.508 & 0.004 & 0.022 & 0.004 \\ 
        "1067685718250692352" & 0.888 & 0.004 & 1.036 & 0.013 & 0.92 & 0.011 & 0.303 & 0.005 \\ 
        "1074883087005896320" & 0.939 & 0.026 & 0.663 & 0.039 & 0.623 & 0.033 & 0.398 & 0.007 \\ 
        "1324699172583973248" & 0.884 & 0.009 & 1.319 & 0.048 & 1.166 & 0.038 & 0.317 & 0.004 \\ 
        "1441993625629660800" & 0.834 & 0.008 & 1.105 & 0.035 & 0.922 & 0.028 & 0.056 & 0.027 \\ 
        "1480959875337657088" & 0.935 & 0.077 & 0.868 & 0.133 & 0.812 & 0.092 & 0.288 & 0.018 \\ 
        "1517219363639758976" & 0.82 & 0.006 & 1.064 & 0.04 & 0.872 & 0.031 & 0.157 & 0.007 \\ 
        "1517927895803742080" & 0.908 & 0.015 & 0.633 & 0.025 & 0.575 & 0.018 & 0.355 & 0.004 \\ 
        "1615450866336763904" & 0.786 & 0.011 & 1.008 & 0.039 & 0.793 & 0.026 & 0.131 & 0.004 \\ 
        "1918953867019478144" & 0.934 & 0.004 & 1.051 & 0.009 & 0.982 & 0.01 & 0.388 & 0.002 \\ 
        "2012218158438964224" & 0.949 & 0.015 & 2.336 & 0.164 & 2.216 & 0.151 & 0.359 & 0.006 \\ 
        "2035577729682322176" & 0.903 & 0.009 & 0.696 & 0.04 & 0.628 & 0.036 & 0.322 & 0.006 \\ 
        "2067948245320365184" & 0.786 & 0.001 & 0.836 & 0.003 & 0.657 & 0.002 & 0.151 & 0.001 \\ 
        "2129771310248902016" & 0.903 & 0.023 & 0.747 & 0.044 & 0.675 & 0.035 & 0.318 & 0.006 \\ 
        "2198442167969655296" & 0.751 & 0.015 & 0.982 & 0.042 & 0.738 & 0.019 & 0.196 & 0.003 \\ 
        "3283823387685219328" & 0.739 & 0.001 & 1.005 & 0.012 & 0.743 & 0.009 & 0.143 & 0.003 \\ 
        "3312631623125272448" & 0.706 & 0.002 & 1.015 & 0.032 & 0.716 & 0.023 & 0.128 & 0.005 \\ 
        "3366718833479009408" & 0.641 & 0.002 & 1.053 & 0.01 & 0.675 & 0.005 & 0.014 & 0.003 \\ 
        "3536759371865789568" & 0.839 & 0.021 & 1.648 & 0.09 & 1.383 & 0.049 & 0.2 & 0.006 \\ 
        "3549833939509628672" & 0.941 & 0.019 & 0.945 & 0.038 & 0.889 & 0.025 & 0.357 & 0.005 \\ 
        "3931519127529822208" & 0.775 & 0.026 & 1.079 & 0.076 & 0.836 & 0.034 & 0.14 & 0.005 \\ 
        "3935131126305835648" & 0.704 & 0.006 & 1.523 & 0.083 & 1.073 & 0.058 & 0.138 & 0.006 \\
        "3954536956780305792" & 0.905 & 0.009 & 1.109 & 1.448 & 1.004 & 1.311 & 0.347 & 0.065 \\ 
        "3964895043508685312" & 0.862 & 0.014 & 0.782 & 0.196 & 0.674 & 0.168 & 0.223 & 0.022 \\ 
        "4228891667990334976" & 0.863 & 0.006 & 1.096 & 0.059 & 0.946 & 0.051 & 0.288 & 0.004 \\ 
        "4354357901908595456" & 0.583 & 0.019 & 0.702 & 0.051 & 0.409 & 0.018 & 0.061 & 0.004 \\ 
        "5762455439477309440" & 0.804 & 0.033 & 0.806 & 0.067 & 0.648 & 0.033 & 0.177 & 0.008 \\ 
        "6244076338858859776" & 0.882 & 0.008 & 0.775 & 0.014 & 0.683 & 0.01 & 0.294 & 0.002 \\ \hline
    \end{tabular}
\end{table*}

\newpage
cc

\newpage


\subsection{GAIA SB2 + GAIA ASTRO}

Calcul direct :
\begin{itemize}
    \item test M1, M2 in [0.1, 5]
    \item test eM1/M1 et eM2/M2 < 0.5
    \item test beta - e-beta < 0.5
\end{itemize}

\begin{table}[!ht]
    \centering
    \begin{tabular}{ccccccccccc}
    \hline
        source\_id & M1 & e-M1 & M1\_up & M1\_low & M2 & e-M2 & M2\_up & M2\_low & Lratio & e-Lratio \\ \hline
        6596891272110663808 & 0.783 & 0.093 & 0.874 & 0.69 & 0.783 & 0.093 & 0.874 & 0.69 & 0.579 & 0.019 \\ \hline
        6344830602266587136 & 1.607 & 0.218 & 1.835 & 1.41 & 1.475 & 0.22 & 1.699 & 1.271 & 0.586 & 0.043 \\ \hline
        6027732067367229312 & 1.139 & 0.033 & 1.17 & 1.106 & 0.97 & 0.029 & 1 & 0.943 & 0.448 & 0.017 \\ \hline
        6017724140678769024 & 0.663 & 0.053 & 0.706 & 0.604 & 0.751 & 0.06 & 0.802 & 0.685 & 0.742 & 0.012 \\ \hline
        5963704000561744768 & 1.437 & 0.101 & 1.545 & 1.343 & 1.748 & 0.115 & 1.876 & 1.646 & 0.615 & 0.027 \\ \hline
        5960988241215882496 & 1.064 & 0.438 & 1.371 & 0.648 & 1.213 & 0.498 & 1.556 & 0.743 & 0.679 & 0.056 \\ \hline
        5583755078792642304 & 0.557 & 0.014 & 0.57 & 0.541 & 0.587 & 0.016 & 0.601 & 0.571 & 0.852 & 0.007 \\ \hline
        5534280594604579584 & 0.8 & 0.021 & 0.82 & 0.778 & 0.955 & 0.026 & 0.98 & 0.929 & 0.598 & 0.011 \\ \hline
        5420408538995944704 & 1.022 & 0.076 & 1.097 & 0.942 & 0.897 & 0.068 & 0.966 & 0.829 & 0.604 & 0.029 \\ \hline
        5116646835246774400 & 0.604 & 0.03 & 0.632 & 0.573 & 0.654 & 0.031 & 0.683 & 0.622 & 0.637 & 0.019 \\ \hline
        5099048571824371712 & 0.551 & 0.047 & 0.598 & 0.502 & 0.53 & 0.042 & 0.572 & 0.488 & 0.316 & 0.018 \\ \hline
        5073754341187667456 & 0.823 & 0.094 & 0.906 & 0.722 & 0.75 & 0.082 & 0.828 & 0.659 & 0.453 & 0.026 \\ \hline
        4940915091531601280 & 0.944 & 0.053 & 0.986 & 0.884 & 0.89 & 0.05 & 0.931 & 0.835 & 0.47 & 0.019 \\ \hline
        4937721834886707584 & 0.652 & 0.117 & 0.761 & 0.529 & 0.621 & 0.111 & 0.727 & 0.504 & 0.51 & 0.036 \\ \hline
        4567743452108176256 & 0.808 & 0.058 & 0.869 & 0.752 & 0.84 & 0.06 & 0.902 & 0.781 & 0.573 & 0.021 \\ \hline
        4503335920679252480 & 0.653 & 0.064 & 0.696 & 0.581 & 0.717 & 0.066 & 0.757 & 0.639 & 0.54 & 0.025 \\ \hline
        4489201252025933696 & 0.617 & 0.034 & 0.652 & 0.583 & 0.725 & 0.049 & 0.773 & 0.679 & 0.398 & 0.025 \\ \hline
        3850933648291811328 & 0.874 & 0.048 & 0.918 & 0.823 & 0.933 & 0.05 & 0.981 & 0.882 & 0.393 & 0.022 \\ \hline
        3487083951918958464 & 0.779 & 0.163 & 0.951 & 0.625 & 0.728 & 0.085 & 0.821 & 0.648 & 0.325 & 0.027 \\ \hline
        3446387075207100032 & 0.492 & 0.066 & 0.559 & 0.435 & 0.631 & 0.084 & 0.715 & 0.557 & 0.402 & 0.029 \\ \hline
        3316189264795366400 & 0.857 & 0.133 & 0.989 & 0.734 & 0.868 & 0.135 & 1.001 & 0.742 & 0.601 & 0.036 \\ \hline
        3304340751399786752 & 0.895 & 0.034 & 0.928 & 0.86 & 0.844 & 0.032 & 0.874 & 0.811 & 0.503 & 0.013 \\ \hline
        3075645223335658240 & 0.463 & 0.063 & 0.525 & 0.406 & 0.447 & 0.062 & 0.512 & 0.39 & 0.75 & 0.045 \\ \hline
        2954775944455492096 & 0.786 & 0.04 & 0.827 & 0.749 & 0.99 & 0.046 & 1.036 & 0.947 & 0.447 & 0.017 \\ \hline
        2921347114487087872 & 0.312 & 0.062 & 0.375 & 0.26 & 0.309 & 0.06 & 0.369 & 0.256 & 0.533 & 0.036 \\ \hline
        2913315010241053696 & 0.586 & 0.028 & 0.6 & 0.557 & 0.575 & 0.027 & 0.588 & 0.549 & 0.854 & 0.014 \\ \hline
        2912325243618165120 & 0.399 & 0.055 & 0.452 & 0.344 & 0.515 & 0.071 & 0.585 & 0.444 & 0.927 & 0.032 \\ \hline
        2767234238970381184 & 1.271 & 0.208 & 1.47 & 1.067 & 1.466 & 0.241 & 1.698 & 1.231 & 0.921 & 0.028 \\ \hline
        2400808142038361088 & 0.315 & 0.045 & 0.363 & 0.274 & 0.369 & 0.035 & 0.406 & 0.337 & 0.64 & 0.034 \\ \hline
        2145277550935525760 & 0.446 & 0.015 & 0.458 & 0.43 & 0.499 & 0.017 & 0.512 & 0.48 & 0.68 & 0.022 \\ \hline
        2035577729682322176 & 0.651 & 0.061 & 0.71 & 0.593 & 0.757 & 0.071 & 0.826 & 0.688 & 0.642 & 0.016 \\ \hline
        1952853322331332864 & 1.125 & 0.075 & 1.201 & 1.05 & 0.816 & 0.064 & 0.881 & 0.752 & 0.247 & 0.021 \\ \hline
        1334277465050081152 & 1.651 & 0.508 & 2.182 & 1.211 & 1.392 & 0.442 & 1.868 & 1.004 & 0.438 & 0.102 \\ \hline
        1205451501554383232 & 0.62 & 0.119 & 0.725 & 0.504 & 0.634 & 0.121 & 0.738 & 0.515 & 0.706 & 0.022 \\ \hline
        1125352388708707840 & 1.819 & 0.164 & 1.967 & 1.642 & 1.597 & 0.142 & 1.72 & 1.437 & 0.581 & 0.023 \\ \hline
        1105311006155685888 & 0.61 & 0.054 & 0.662 & 0.558 & 0.562 & 0.05 & 0.611 & 0.513 & 0.64 & 0.015 \\ \hline
        1097717538333601408 & 0.987 & 0.049 & 1.034 & 0.938 & 1.295 & 0.065 & 1.358 & 1.23 & 0.452 & 0.017 \\ \hline
        1067685718250692352 & 1.002 & 0.047 & 1.047 & 0.955 & 0.869 & 0.041 & 0.908 & 0.827 & 0.411 & 0.012 \\ \hline
        1017645329162554752 & 1.049 & 0.289 & 1.323 & 0.851 & 1.122 & 0.309 & 1.416 & 0.906 & 0.888 & 0.025 \\ \hline
        1012707766039635968 & 0.525 & 0.024 & 0.549 & 0.501 & 0.533 & 0.025 & 0.558 & 0.508 & 0.397 & 0.019 \\ \hline
        843086760057866240 & 0.671 & 0.145 & 0.797 & 0.552 & 0.688 & 0.149 & 0.818 & 0.565 & 0.619 & 0.03 \\ \hline
        596187575750053504 & 0.59 & 0.128 & 0.724 & 0.461 & 0.554 & 0.116 & 0.665 & 0.438 & 0.625 & 0.075 \\ \hline
        595390807776621824 & 0.759 & 0.021 & 0.778 & 0.738 & 0.894 & 0.024 & 0.917 & 0.871 & 0.633 & 0.008 \\ \hline
        466178297230210816 & 0.919 & 0.042 & 0.961 & 0.88 & 0.909 & 0.042 & 0.95 & 0.871 & 0.747 & 0.018 \\ \hline
        458543563370852096 & 0.663 & 0.062 & 0.719 & 0.595 & 0.606 & 0.055 & 0.655 & 0.546 & 0.298 & 0.03 \\ \hline
        423764017715132544 & 2.67 & 0.121 & 2.792 & 2.552 & 4.208 & 0.165 & 4.375 & 4.05 & 0.912 & 0.024 \\ \hline
    \end{tabular}
\end{table}

\newpage
coucou
\newpage

\subsection{CARMENES SB2 + GAIA ASTRO}

\begin{table}[!ht]
    \caption{Gaia + CARMENES}
    \label{table:3}
    \centering
    \begin{tabular}{cccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID & $M_1$ & $M_1~up$ & $M_1~low$ & $M_2$ & $M_2~up$ & $M_2~low$ & $LR$ & $LR~up$ & $LR~low$ \\ \hline \hline
        PB MUP < M : 308256610357824640 & 0.44 & 0.243 & 0.051 & 0.312 & 0.171 & 0.036 & 0.395 & 0.331 & 0.166 \\ 
        3427930123268526720 & 0.933 & 1.202 & 0.695 & 0.308 & 0.397 & 0.231 & 0.079 & 0.099 & 0.062 \\ \hline
    \end{tabular}
\end{table}


\begin{table}[!ht]
    \caption{Gaia + CARMENES V2}
    \label{table:3}
    \centering
    \begin{tabular}{cccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID & $M_1$ & $M_1~up$ & $M_1~low$ & $M_2$ & $M_2~up$ & $M_2~low$ & $LR$ & $LR~up$ & $LR~low$ \\ \hline \hline
        308256610357824640 & 0.445 & 0.514 & 0.174 & 0.315 & 0.365 & 0.123 & 0.395 & 0.408 & 0.308 \\
        3427930123268526720 & 0.955 & 1.048 & 0.868 & 0.316 & 0.346 & 0.287 & 0.081 & 0.088 & 0.074 \\ \hline
    \end{tabular}
\end{table}

\begin{table}[!ht]
    \caption{Gaia + CARMENES V3}
    \label{table:3}
    \centering
    \begin{tabular}{cccccccccc}
    \hline \hline
        GAIA DR3 Source\_ID & $M_1$ & $M_1~up$ & $M_1~low$ & $M_2$ & $M_2~up$ & $M_2~low$ & $LR$ & $LR~up$ & $LR~low$ \\ \hline \hline
        308256610357824640 & 0.445 & 0.51 & 0.173 & 0.315 & 0.361 & 0.123 & 0.395 & 0.407 & 0.305 \\
        3427930123268526720 & 0.955 & 1.055 & 0.879 & 0.316 & 0.349 & 0.291 & 0.081 & 0.089 & 0.075 \\ \hline
    \end{tabular}
\end{table}


